SinGRAV: Learning a Generative Radiance Volume from a Single Natural Scene

We present a 3D generative model for general natural scenes. Lacking necessary volumes of 3D data characterizing the target scene, we propose to learn from a single scene. Our key insight is that a natural scene often contains multiple constituents whose geometry, texture, and spatial arrangements follow some clear patterns, but still exhibit rich variations over different regions within the same scene. This suggests localizing the learning of a generative model on substantial local regions. Hence, we exploit a multi-scale convolutional network, which possesses the spatial locality bias in nature, to learn from the statistics of local regions at multiple scales within a single scene. In contrast to existing methods, our learning setup bypasses the need to collect data from many homogeneous 3D scenes for learning common features. We coin our method SinGRAV, for learning a Generative RAdiance Volume from a Single natural scene. We demonstrate the ability of SinGRAV in generating plausible and diverse variations from a single scene, the merits of SinGRAV over state-of-the-art generative neural scene methods, as well as the versatility of SinGRAV by its use in a variety of applications, spanning 3D scene editing, composition, and animation. Code and data will be released to facilitate further research.

==> 3-method-back.tex <==
\section{Method}

\input{math_utils}

% yujie: In this overview, we should point out:
%1) we use 3d convolutional neural networks since it supports local patch learning.
%2）our supervision is in image domain, which demands us to use volume rendering for projecting the
%3d scene to the image domain. 
% Why do we impose supervisions in the image domain? (briefly introduce them into the introduction section)
%I would say:
%(2.1) image data is much more easier to be obtained than precise 3d models (due to the limitations of current 3d reconstruction techniques)
%(2.2) directly supervising the image domain contributes to a guarantee of high quality of the generated views with limited data volume budget. (the budget is especially severe when we are using the volume as representation.) (ps: Actually, current MLP based solutions are also unable to directly produce high resolution results.)
% In the supplementary file, we may want to demonstrate that we have no need to use perfect depth for training, which makes the method more practical.

\name learns a powerful generative radiance volume from multi-view images $\imset = \{ \im^1, ..., \im^{m} \} $ of a single input scene, where $m$ denotes the number of images.
In contrast to training over many class-specific scenes for learning common features,
our specific emphasis here is to learn from a variety of local regions within the single scene,
%The key difference is that the training samples are those 3D patches.
implying the key is to localize the learning. 
Hence, we deviate from popular continuous MLP-based neural scene representations, and in turn resort to a convolutional network architecture, in which 3D convolutional operations possessing spatial locality bias are adopted for generating discrete radiance volumes. \yujie{The variants adopting MLP-based coordinate neural representations will be discussed in our ablation study in Section \ref{sec:ablation}.} Due to the limited data volume budeget of the hardwares, we direclty carry supervions in the image domain, for which we leverage volume rendering to render 2D images from the generated scenes.
%and the adversarial discrimination is performed on 2D though a differentiable renderer.
Moreover,
%similar in spirit with SinGAN, 
we use a hybrid and multi-scale learning framework to learn properties at different scales, ranging from global configurations to local fine texture details.
In the following, we start elaborating the data representation, network architecture and training scheme.

\input{figure_framework}
\subsection{Neural radiance volume and rendering}

%\paragraph{Neural radiance volume.}
We assume the generated scene can be modeled as a discrete 3D grid of voxels, which is produced as the output of a 3D convolutional network.
Each voxel center stores a 4-channel vector that contains a density scalar $\density$ and a color vector $\rgb$. Trilinear interpolation is used to define a continuous radiance field throughout the whole volume.
Formally, given a sampling coordinate, the radiance volume returns a trilinear-interpolated vector $V: \xyz \rightarrow (\rgb, \density)$.

%\paragraph{Volume rendering.}
We use the same differentiable function as in NeRF~\cite{nerf} for volume rendering generated radiance volumes.
The expected color $\hat{C}$ of a camera ray $\ray$ is approximated by integrating over $M$ samples spreading along the ray:
\begin{equation} 
    \begin{gathered}
        \hat{C}{(\ray)} = \sum_{i=1}^{M} T_i \big( 1 - \expo(-\density_i \delta_i) \big) \rgb_i,
        \; \text{and} \; T_i = \expo\Big( -\sum_{j=1}^{i-1}\density_j \delta_j \Big),
    \end{gathered}
\end{equation}
where
the subscript denotes the index of samples between near and far bounds $t_n$ and $t_f$,
$\delta_i = t_{i+1} - t_i$ is the distance between two consecutive samples,
and \yujie{$T_i$ is the accumulated transmittance at sample $i$, which is obtained via integrating over the preceding samples along the ray.}
This color rendering is reduced to traditional alpha compositing with alpha values $\alpha_i = 1 - \expo(-\density_i \delta_i)$.
This function is differentiable and enables updating the 3D representation based on the error derived from the supervision signals.

\subsection{Hybrid multi-scale architecture}
Our model is similar in spirit with SinGAN\cite{singan}, consisting of a pyramid of 3D convolutional generators, $ \Gset = \{ \G_\scale \}$, $\scale=\{ 1,...,N \}$, for progressively generating a volume with higher resolutions at $N$ different scales.
The volume resolution increases by a factor of $\theta$ between two consecutive scales.
Specially, to address the overly high computing cost, the last 3D generator retains the volume resolution from previous scale and is paired with a lightweight 2D convolutional generator $G_{N}^{2D}$ for higher-resolution renderings.
%
All generators are trained with supervision from a downsampled version  $\imset_\scale = \{ \im^1_\scale, ..., \im^{m}_\scale \}$ of the input image set $\imset$ by a factor of $\eta^{N-\scale}$ at the corresponding $\scale$-th scale,
to progressively model a volume that is realistic w.r.t the distribution of regions in the input scene.
%The image resolution increases by a factor of by $\eta$  between two consecutive scales.
%
%The 3D convolutional generators are trained to progressively model a volume with structural variations that are realistic w.r.t the distribution of regions in the input scene, 
%while the 2D convolutional generator at the finest scale is trained to enhance the rendering from previous scale with finer texture variations that are realistic w.r.t the patch distribution in the input images.
%
The model is learned through the differentiable renderer and adversarial training, where $G_\scale$ learns to generate realistic volumes that can be rendered to fool an associated 2D discriminator $D^{2D}_\scale$, which attempts to distinguish patches in the generated renderings from patches in $\imset_s$.
Note, in particular, we do \emph{NOT} employ 3D discriminators for directly supervising the 3D volume, as we observed minor benefits and significantly slow training speed.

%\paragraph{3D volume generation.}
The generation starts with modeling a 3D volume at the coarsest scale and sequentially passes through all generators for higher volume resolutions up to the finest scale,with noise injection at each scale.
At the coarsest scale, the volume generation is purely generative, i.e.\ $G_1$ maps a spatial white Gaussian noise volume $z_1$ to an radiance volume.
Importantly, positional-encoded information has been proofed to be crucial in many coordinate-based models. 
Thus, we create a positional encoding volume $p_1$ which stores the center coordinate of each voxel in the normalized Cartesian Spatial Grid (CSG)~\cite{csg_singan}, and feed it to $G_1$:
\begin{equation} 
    \begin{gathered}
        \volgen_1 = G_1(z_1, p_1).
    \end{gathered}
\end{equation}
Specially, $p_1$ is added to the noise volume $z_1$.
We only inject the positional encoding volume at the coarsest scale, 
as the positional-encoded information will be propagated throughout the convolution operations and affect the subsequent training~\cite{csg_singan}.
The effective receptive field of the generator and the discriminator at this scale is typically around $1/2$ of the volume of interest and the image size,
thus $G_1$ learns to generate the overall layout and structure of the objects in the scene.

Subsequently, each generator $G_\scale$ at finer scales ($1<\scale<N$) learns to add details that are missing from previous scale.
Hence, each generator $G_\scale$ takes as input a spatial noise volume $z_\scale$, along with an upsampled version of the volume $(\volgen_{\scale-1}) \uparrow^{\theta}$ generated from the coarser scale:
Specially, prior to being fed into $G_\scale$, the noise $z_\scale$ is added to the volume $(\volgen_{\scale-1}) \uparrow^{\theta}$,
and, akin to residual learning~\cite{residual}, $G_\scale$ only learns to generate missing details in $(\volgen_{\scale-1}) \uparrow^{\theta}$:
\begin{equation} 
    \begin{gathered}
        \volgen_\scale = (\volgen_{\scale-1}) \uparrow^{\theta} + \; G_\scale \big( z_\scale, (\volgen_{\scale-1}) \uparrow^{\theta} \big),\; 1 < \scale < N.
    \end{gathered}
\end{equation}

% 2D 3D consistency? receptive field?
%a very key choise: 
%All 3D generators and the associated 2D discriminators have the same receptive field, and thus learn to capture structures of smaller size as the volume resolution goes up in the generation process.
%\paragraph{2D enhancement scale.}
At the finest scale, 
$G_{N}$ retains the the volume resolution from previous scale and instead generates a feature volume $\volgen^{f}_{N}$ from the noise $z_N$. 
A feature map $f_N$ can then be aggregated via volume rendering from a given viewpoint.
Last, a 2D convolutional generator $\Gtwod_{N}$ takes as input the concatenation of $f$ and the rendering $\imgen_{N-1}$ produced from the generated radiance volume at previous scale,
and enhances the final rendering with more details:
\begin{equation} 
    \begin{gathered}
        \imgen_N = \Gtwod_N ( \imgen_{N-1}, f_N ).
    \end{gathered}
\end{equation}
Note $\Gtwod_N$ employs upsampling layers as in~\cite{stylenerf}, and thus produces the final image that twice the resolution of $\imgen_{N-1}$.


\subsection{Training}
The multi-scale network architecture is sequentially trained, from the coarsest to the finest scale.
The GANs at coarser scales are freezed once trained.
The loss for training GAN at the $n$-th scale consists of an adversarial term and a reconstruction term as in~\cite{singan}:
\begin{equation} 
    \begin{gathered}
        \min_{G_\scale} \max_{D_\scale^{2D}}  \loss_{adv}(G_\scale, D_\scale^{2D}) + \alpha \loss_{rec}(G_\scale).
    \end{gathered}
\end{equation}

view, depth used in discriminators
depth used in recon loss


\subsection{Test}




==> ack.tex <==
\section{Acknowledgments}

Identification of funding sources and other support, and thanks to
individuals and groups that assisted in the research and the
preparation of the work should be included in an acknowledgment
section, which is placed just before the reference section in your
document.

This section has a special environment:
\begin{verbatim}
  \begin{acks}
  ...
  \end{acks}
\end{verbatim}
so that the information contained therein can be more easily collected
during the article metadata extraction phase, and to ensure
consistency in the spelling of the section heading.

Authors should not prepare this section as a numbered or unnumbered {\verb|\section|}; please use the ``{\verb|acks|}'' environment.

==> author.tex <==
% %%
% %% The "author" command and its associated commands are used to define
% %% the authors and their affiliations.
% %% Of note is the shared affiliation of the first two authors, and the
% %% "authornote" and "authornotemark" commands
% %% used to denote shared contribution to the research.
% \author{Ben Trovato}
% \authornote{Both authors contributed equally to this research.}
% \email{trovato@corporation.com}
% \orcid{1234-5678-9012}
% \author{G.K.M. Tobin}
% \authornotemark[1]
% \email{webmaster@marysville-ohio.com}
% \affiliation{%
%   \institution{Institute for Clarity in Documentation}
%   \streetaddress{P.O. Box 1212}
%   \city{Dublin}
%   \state{Ohio}
%   \country{USA}
%   \postcode{43017-6221}
% }

% \author{Lars Th{\o}rv{\"a}ld}
% \affiliation{%
%   \institution{The Th{\o}rv{\"a}ld Group}
%   \streetaddress{1 Th{\o}rv{\"a}ld Circle}
%   \city{Hekla}
%   \country{Iceland}}
% \email{larst@affiliation.org}

% \author{Valerie B\'eranger}
% \affiliation{%
%   \institution{Inria Paris-Rocquencourt}
%   \city{Rocquencourt}
%   \country{France}
% }

% \author{Aparna Patel}
% \affiliation{%
%  \institution{Rajiv Gandhi University}
%  \streetaddress{Rono-Hills}
%  \city{Doimukh}
%  \state{Arunachal Pradesh}
%  \country{India}}

% \author{Huifen Chan}
% \affiliation{%
%   \institution{Tsinghua University}
%   \streetaddress{30 Shuangqing Rd}
%   \city{Haidian Qu}
%   \state{Beijing Shi}
%   \country{China}}

% \author{Charles Palmer}
% \affiliation{%
%   \institution{Palmer Research Laboratories}
%   \streetaddress{8600 Datapoint Drive}
%   \city{San Antonio}
%   \state{Texas}
%   \country{USA}
%   \postcode{78229}}
% \email{cpalmer@prl.com}

% \author{John Smith}
% \affiliation{%
%   \institution{The Th{\o}rv{\"a}ld Group}
%   \streetaddress{1 Th{\o}rv{\"a}ld Circle}
%   \city{Hekla}
%   \country{Iceland}}
% \email{jsmith@affiliation.org}

% \author{Julius P. Kumquat}
% \affiliation{%
%   \institution{The Kumquat Consortium}
%   \city{New York}
%   \country{USA}}
% \email{jpkumquat@consortium.net}

% %%
% %% By default, the full list of authors will be used in the page
% %% headers. Often, this list is too long, and will overlap
% %% other information printed in the page headers. This command allows
% %% the author to define a more concise list
% %% of authors' names for this purpose.
% \renewcommand{\shortauthors}{Trovato and Tobin, et al.}

\author{Yujie Wang}
\affiliation{%
  \institution{Shandong University and Peking University}
  %\streetaddress{30 Shuangqing Rd}
  \city{Qingdao}
  \state{Shandong}
  \country{China}}
  
 \author{Xuelin Chen}
\affiliation{%
  \institution{Tecent AI lab}
  %\streetaddress{30 Shuangqing Rd}
  \city{Shenzhen}
  \state{Guangdong}
  \country{China}}
  
 \author{Baoquan Chen}
\affiliation{%
  \institution{Peking University}
  %\streetaddress{30 Shuangqing Rd}
  \city{Beijing}
  \state{Beijing}
  \country{China}}

==> figure_application.tex <==
\if 0
\setlength{\tabcolsep}{1pt}
\renewcommand{\arraystretch}{1}
\begin{figure*}[t]
\begin{center}

\begin{tabular}{cc}
\vspace{-0.4mm}
%  \small{Retargeting} & \small{Composition} \\
\makebox[0.42\textwidth][c]{\small{Retargeting}} & \small{Composition} \\
\multicolumn{2}{c}{\includegraphics[width=\linewidth]{image/figure_app2.pdf}}\\
\vspace{-4mm}
\end{tabular}
\end{center}
\caption{Results for retargeting (Left) and scene editing (Right). Three viewpoints are provided for the composited scene.}
 \label{fig:apps}
\end{figure*}

\fi

==> figure_real_candle.tex <==
\setlength{\tabcolsep}{1pt}
\renewcommand{\arraystretch}{1}
\begin{figure*}[t]
\begin{center}

\begin{tabular}{cc}
\vspace{-0.4mm}
\makebox[0.25\textwidth][c]{\small{Training scene}} & \small{Random generation} \\
\multicolumn{2}{c}{\includegraphics[width=\linewidth]{image/figure_real_candle.pdf}}\\
\vspace{-7mm}
\end{tabular}
\end{center}
\caption{Another example for generation on candles.} 
 \label{fig:candle}
\end{figure*}

==> supp_materials/algorithm1.tex <==
\RestyleAlgo{ruled}
\begin{algorithm}[hbt!]
\caption{Training process at scale $s$.}\label{alg:supp}
% \KwData{$n \geq 0$}
% \KwResult{$y = x^n$}
% \textbf{Input: $\{z_{\scale}\}_{\scale=1}^{s}$} \\
\textbf{Input:} noise volume sequence $\{z_{\scale}\}_{\scale=1}^{s}$ \\ 
\textbf{Output:} generated volume $\tilde{V}_{s}$, rendered image $\tilde{x}_{\scale}$ and depth $\tilde{d}_{\scale}$ \\
\textbf{Parameters:} parameters in $G_{s}$ and $D_{s}$ \\
\While{$i<T$}
{
    \eIf{$i<T_1$}
    {
        optimize $G_s$ with $\loss_{rec}$ according to $\loss_{rec}$ Eq.(\ref{eq:loss_rec});
    }
    {
    \eIf{$J<D_{steps}$}{
       $\tilde{V}_s = \{G_{\scale}\}_{\scale=1}^{s}(\{z_{\scale}\}_{\scale=1}^{s},e_1)$;\\
       $\tilde{x}_s=\pi(\tilde{V}_s)$;
    }{
    }
        optimize $G_s$ and $D_s$ according to the loss given in Eq. (\ref{eq:loss_total});
    }
}
% $y \gets 1$\;
% $X \gets x$\;
% $N \gets n$\;
% \While{$N \neq 0$}{
%   \eIf{$N$ is even}{
%     $X \gets X \times X$\;
%     $N \gets \frac{N}{2} $ \Comment*[r]{This is a comment}
%   }{\If{$N$ is odd}{
%       $y \gets y \times X$\;
%       $N \gets N - 1$\;
%     }
%   }
% }
\end{algorithm}

==> table_ablation.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet3'
\begin{table}[b!]
\small
  \centering
  \caption{Numerical results for variants of \name.}
    \begin{tabular}{lccc}
    \toprule
    Variant & Image resolution & SIFID-MV $\downarrow$ & Diversity-MV $\uparrow$ \\
    \midrule
    \name (wo. CSG) & $320\times320$ & 0.1307 & \textbf{0.8434} \\
    \name (wo. SWD) & $320\times320$ & 0.2713 & 0.7730 \\
    \name (wo. depth sup.) & $320\times320$ & 0.1157 & 0.7910 \\
    \name (NeRF-recon. depth)  & $320\times320$ & 0.1290 7 0.8046 \\
    \name (self-recon. depth) &  & $320\times320$ & 0.1120 & 0.7862 \\
    \name (MLP) & $160\times160$ & 0.1843 & 0.5235 \\
    \name (MLP-LLG) & $108\times108$ & 0.2013 & 0.4621 \\
    % \name (resize)  & $160\times160$ & 0.1770 & 0.7585 \\  % remove this since resize is not fair for a network trained on 320x320, resizing will introduce extra differences into the distributions.
     \name  & $320\times320$ & \textbf{0.1113} & 0.7769 \\ 
    \bottomrule
    \end{tabular}%
  \label{tab:ablation}%
\end{table}%



==> table_ablation_depth.tex <==
% % Table generated by Excel2LaTeX from sheet 'Sheet3'
% \begin{table}[b!]
% \small
%   \centering
%   \caption{Numerical results for using imperfect depth.}
%     \begin{tabular}{lccc}
%     \toprule
%     Variant & Image resolution & SIFID-MV $\downarrow$ & Diversity-MV $\uparrow$ \\
%     \midrule
%     \name (wo. CSG) & $320\times320$ & 0.1307 & \textbf{0.8434} \\
%     \name (wo. SWD) & $320\times320$ & 0.2713 & 0.7730 \\
%     \name (wo. Depth sup.) & $320\times320$ & 0.1157 & 0.7910 \\
%     \name (MLP) & $160\times160$ & 0.1843 & 0.5235 \\
%     \name (MLP-LLG) & $108\times108$ & 0.2013 & 0.4621 \\
%     % \name (resize)  & $160\times160$ & 0.1770 & 0.7585 \\  % remove this since resize is not fair for a network trained on 320x320, resizing will introduce extra differences into the distributions.
%      \name  & $320\times320$ & \textbf{0.1113} & 0.7769 \\ 
%     \bottomrule
%     \end{tabular}%
%   \label{tab:ablation_depth}%
% \end{table}%



% % Table generated by Excel2LaTeX from sheet 'ablation depth'
 \setlength{\tabcolsep}{5.5pt}
\begin{table*}[htbp]
\scriptsize
\centering
\caption{Performance for training with multi-view RGB observations.}
\begin{tabular}{lcccc}
% \begin{tabular}{>{\color{blue}}l >{\color{blue}}c >{\color{blue}}c >{\color{blue}}c >{\color{blue}}c }

\toprule
\multicolumn{1}{c}{\multirow{2}[4]{*}{Variant}} & \multicolumn{2}{c}{\emph{Stonehenge}} & \multicolumn{2}{c}{\emph{Grass and flower}} \\
\cmidrule{2-5} &  \multicolumn{1}{l}{SIFID-MV $\downarrow$} & \multicolumn{1}{l}{Diversity-MV $\uparrow$} & \multicolumn{1}{l}{SIFID-MV $\uparrow$} & \multicolumn{1}{l}{Diversity-MV  $\downarrow$} \\
\midrule
SinGRAV (self-recon. depth) & 0.0590 & 0.7323 & 0.2070 & 1.0008 \\
SinGRAV (NeRF-recon. depth) & 0.0680 & $\mathbf{0.7756}$ & 0.2490 & $\mathbf{1.0059}$ \\
SinGRAV & $\mathbf{0.0550}$ & 0.7281 & $\mathbf{0.2010}$ & 0.9787 \\
\bottomrule
\end{tabular}%
\label{tab:ablation_depth}%
\end{table*}%

==> table_comparison.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet5'
\begin{table}[b!]
\small
  \centering
  \caption{
  Quantitative comparisons.
  Top two on each metric are highlighted.
  All baselines suffer from severe mode collapse, producing low scores on Diversity-MV,
  while
  \name presents diverse scenes that are meanwhile visually similar to the input training scene.
  }
    \begin{tabular}{lccc}
    \toprule
    Method & Image resolution & SIFID-MV $\downarrow$ & Diversity-MV $\uparrow$ \\
    \midrule
    GRAF   & $320\times320$ & 0.4447 & 0.1337 \\
    pi-GAN  & $128\times128$ & \textbf{0.0133} & 0.1157 \\
    GIRAFFE  & $320\times320$ & 0.4710      & \textbf{0.3198} \\
    %%MLGSN \cite{unconstrained} & $128\times128$ &       &  \\
    % \name (resize)  & $128\times128$ &       &  \\
    \name  & $320\times320$ & \textbf{0.1113} & \textbf{0.7769} \\
    \bottomrule
    \end{tabular}%
  \label{tab:comparison}%
\end{table}%




% % Table generated by Excel2LaTeX from sheet 'Sheet5'
% \begin{table}[b!]
% \small
%   \centering
%   \caption{
%   Quantitative comparisons.
%   Top two on each metric are highlighted.
%   All baselines suffer from severe mode collapse, producing low scores on Diversity-MV,
%   while
%   \name presents diverse scenes that are meanwhile visually similar to the input training scene.
%   }
%     \begin{tabular}{lccc}
%     \toprule
%     Method & Image resolution & SIFID-MV $\downarrow$ & Diversity-MV $\uparrow$ \\
%     \midrule
%     GRAF \cite{graf}  & $320\times320$ & 0.4447 & 0.1337 \\
%     pi-GAN \cite{pi-gan} & $128\times128$ & \textbf{0.0133} & 0.1157 \\
%     GIRAFFE \cite{giraffe} & $320\times320$ & 0.4710      & \textbf{0.3198} \\
%     %%MLGSN \cite{unconstrained} & $128\times128$ &       &  \\
%     % \name (resize)  & $128\times128$ &       &  \\
%     \name  & $320\times320$ & \textbf{0.1113} & \textbf{0.7769} \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:comparison}%
% \end{table}%





